Receding Horizon Iterative Learning Control for Continuously Operated Systems

This paper presents an iterative learning control (ILC) scheme for continuously operated repetitive systems for which no initial condition reset exists. To accomplish this, we develop a lifted system representation that accounts for the effect of the initial conditions on dynamics and projects the dynamics over multiple future iterations. Additionally, we develop an economic cost function and update law that considers the performance over multiple iterations in the future, thus allowing for the prediction horizon to be larger than just the next iteration. Convergence of the iteration varying initial condition and applied input are proven and demonstrated using a simulated servo-positioning system test case.

==> IEEETran/README <==

August 26, 2015


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.

 2. The \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later.

 3. The \IEEEnoauxwrite command.

 4. The IEEE itemize, enumerate and description list environments.

 5. The complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

 6. The \IEEEQEDhere and \IEEEQEDhereams commands to provide amsthm.sty
    \qedhere functionality to IEEEproof. \IEEEQEDhere is for simple use
    "right on the spot" such as within an IEEEeqnarry:

    \begin{IEEEproof}
       \begin{IEEEeqnarray}{rCl+x*}
        x & = & y & \nonumber\IEEEQEDhere
       \end{IEEEeqnarray}
    \end{IEEEproof}

    While \IEEEQEDhereams is like amsthm's venerable \qedhere and is
    for use within the standard equation environment:

    \begin{IEEEproof}
     \begin{equation}
       x = y \nonumber\IEEEQEDhereams\quad
     \end{equation}
    \end{IEEEproof}

    Note that the qedhere style is normally not done with IEEE-related
    work so these are undocumented features of IEEEtran.cls.

    Thanks Mark D. Butala, Hennadiy Leontyev and Stefan M. Moser for
    suggesting this feature.



IEEEtrantools.sty is not needed and should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
2015/08/26 V1.5 (V1.8b of IEEEtran.cls) changes:

 1) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 2) Fix bug with IEEEeqnarray equation number foreground color
    under the color environment of Beamer class.
    Thanks to Joschi Brauchle for reporting this problem.

 3) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.



********************************** Files **********************************

README                - This file.

changelog.txt         - The revision history.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> sections/OptimalLearningFilters.tex <==
\subsection{Receding Horizon Iterative Learning Control}\label{sec:RHILC}

For many systems, it is suboptimal or infeasible to reset the initial conditions of the system between iterations.  In systems without an initial condition reset, the control sequence chosen for one iteration has a direct impact on subsequent iterations.  Therefore to optimize the control sequence, we must account for this interdependence.  To capture this interdependence, we first develop a dynamic model to capture the behavior of the system over multiple future iterations.  We then use that dynamic model to estimate the performance of the system over multiple future iterations.  We can then use that estimate of performance to derive learning filters.

The procedure for deriving the update law and learning filters is similar to other works such as \cite{p2p4}.  First, we write a performance index in terms of the lifted model, then we take the gradient of that performance index and set it equal to the zero vector, rearranging the result to obtain an update law and expressions for learning filters.

To clarify the following math and notation, we wish to define a standard of notation and nomenclature to differentiate symbols and quantities.  In previous sections, we refer to $\underline{x}_j$ and $\underline{u}_j$ as ``lifted'' vectors.  That is, they are formed by concatenating a set of state or control input vectors ordered according to their path position (or time stamp) as in \eqref{eqn:liftedVectors}.  We also referred to the matrices $G_j$ and $F_j$ as ``lifted'' system matrices. In this section, it will be necessary to concatenate multiple instances of vectors and matrices that are already lifted.  We refer to these further concatenated vectors and block matrices as ``super-lifted'' to emphasize that they are different from but dependent upon vectors and matrices from the previous section which themselves are already lifted.  These super-lifted vectors and matrices will be notated with a bold-faced symbol.

In general, the lifted model of \eqref{eqn:liftedModel} can be used to predict the state sequence resulting from any control input.  Thus, if we wish to predict the state sequence over the $(j+n_i)^{\mathrm{th}}$ iteration, we could write
\begin{equation} \label{eqn:generalLiftedModel}
    \underline{x}_{j+n_i} = \underline{x}_j +G_j\left( \underline{u}_{j+n_i} - \underline{u}_j \right) + F_j \left( E_F - E_I\right) \underline{x}_{j+n_i-1}.
\end{equation}
Noting the recursive form of this relationship, ($\underline{x}_{j+n_i}$ depends on $\underline{x}_{j+n_i-1}$), we can use it to derive a relationship between the super-lifted state and control vectors, $\mathbf{x}_{j+1}$ and $\mathbf{u}_{j+1}$, which are defined as 
\begin{align}
\mathbf{x}_{j+1} \triangleq \begin{bmatrix} \underline{x}_{j+1} \\ \underline{x}_{j+2} \\ \vdots \\ \underline{x}_{j+N_i-1} \\ \underline{x}_{j+N_i}\end{bmatrix}, \quad \mathrm{and} \quad
\mathbf{u}_{j+1} \triangleq \begin{bmatrix} \underline{u}_{j+1} \\ \underline{u}_{j+2} \\ \vdots \\ \underline{u}_{j+N_i-1} \\ \underline{u}_{j+N_i}\end{bmatrix},
\end{align}
respectively.  The relationship between $\mathbf{x}_{j+1}$ and $\mathbf{u}_{j+1}$ is then given as 
\begin{align}\label{eqn:superLiftedModel}
\mathbf{x}_{j+1} = \left(\mathbf{I}_x +\mathbf{F}_j \right)x_j + \mathbf{G}_j \left(\mathbf{u}_{j+1} - \mathbf{I}_u u_j \right)
\end{align}
where
\begin{equation}
    \mathbf{F}_j \triangleq \begin{bmatrix} \mathbb{I} \\ \mathbb{I} + F_j E_F \\ \vdots \\ \mathbb{I} + \sum\limits_{k = 1}^{N_i-1} \prod\limits_{m=1}^{k}F_j E_F \\ \mathbb{I} + \sum\limits_{k = 1}^{N_i} \prod\limits_{m=1}^{k}F_j E_F \end{bmatrix},
\end{equation}

\begin{equation}
    \mathbf{G}_j \triangleq \tiny
    \begin{bmatrix} 
G_j & \mathbb{0}            & \hdots    & \hdots        & \mathbb{0} \\
F_j E_F G_j   & G_j         & \hdots    & \hdots        & \mathbb{0} \\
\vdots & \vdots & \vdots & \ddots & \vdots \\
\left(\prod\limits_{m=1}^{N_i-1}F_j E_F\right)G_j & \left(\prod\limits_{m=1}^{N_i-2}F_j E_F\right)G_j & \hdots & G_j & \mathbb{0} \\
\left(\prod\limits_{m=1}^{N_i}F_j E_F\right)G_j & \left(\prod\limits_{m=1}^{N_i-1}F_j E_F\right)G_j & \hdots & F_j E_F G_j & G_j
\end{bmatrix}
\normalsize
\end{equation}

\noindent and $\mathbf{I}_{(\cdot)}$ is defined as an appropriately sized identity matrix, $\mathbb{I}^{n_{(\cdot)} ns \times n_{(\cdot)} ns}$, repeated vertically, $N_i$ times.  Similarly, we can calculate a super-lifted error vector as 
\begin{equation}\label{eqn:liftedError}
    \mathbf{e}_{j+1}  = \mathbf{I}_r \underline{r} - \mathbf{x}_{j+1}
\end{equation}
where $\underline{r}$ is the lifted reference signal vector constructed from an ordered set of reference states, $\{r_0,\, r_1,\,\hdots ,\,,r_{n_s-1},r_{n_s} \}$ where $r_q\in \mathbb{R}^{n_x}$ according to the same method as shown in \eqref{eqn:liftedVectors}.

Here, we assume that at every point along the path (or in time), there is a reference state, $r$, with the same number of elements as $x$.  In practice, however, one can build a reference state vector that contains the desired values of the states for only at the indices considered by the tracking penalty in the subsequent learning filters.

We then select the following general form of performance index:
\begin{equation}\label{eqn:longFormPerformance}
\begin{split}
\mathbf{J}_{j+N} 
\!\!=\!\! \sum_{k=1}^{N}(
& \underline{u}_{j\!+\!k}^T \!Q_u\! \underline{u}_{j\!+\!k} \!\!+\!\! \left(\underline{u}_{j\!+\!k}\!\!-\!\!\underline{u}_{j\!+\!k\!-\!1}\right)^T \!\!Q_{\delta u}\! \left(\underline{u}_{j\!+\!k}\!\!-\!\!\underline{u}_{j\!+\!k\!-\!1}\right) \\
& +\!\! \underline{x}_{j\!+\!k}^T \!Q_x\! \underline{x}_{j\!+\!k} \!\!+\!\! \left(\underline{x}_{j\!+\!k}\!\!-\!\!\underline{x}_{j\!+\!k\!-\!1}\right)^T \!\!Q_{\delta x}\! \left(\underline{x}_{j\!+\!k}\!\!-\!\!\underline{x}_{j\!+\!k\!-\!1}\right) \\
& +\!\!\underline{e}_{j\!+\!k}^T \!Q_e\! \underline{e}_{j\!+\!k} \!\!+\!\! \left(\underline{e}_{j\!+\!k}\!\!-\!\!\underline{e}_{j\!+\!k\!-\!1}\right)^T \!\!Q_{\delta e}\! \left(\underline{e}_{j\!+\!k}\!-\!\underline{e}_{j\!+\!k\!-\!1}\right) \\
& + S_x x_{j\!+\!k}).
\end{split}
\end{equation}
The diagonal positive definite weighting matrices of the quadratic terms, $Q_u$, $Q_{\delta u}$, $Q_x$, $Q_{\delta x}$, $Q_e$, and $Q_{\delta e}$ are defined in detail in appendix \ref{apn:perfIndexWeights}, but they follow the standard norm-optimal point-to-point structure detailed in other work such as \cite{p2p4}. 

In order to accommodate economic objectives, we introduce the last term of \eqref{eqn:longFormPerformance}.  The quantity $S_x\in \mathbb{R}^{n_x n_s}$ here is taken to be a weighted linear approximation (or exact representation) of the true economic objective that the user would like to optimize.  If the economic objective is described by $J_e(\underline{x},\underline{u})$, then 
\begin{equation}
    S_x \triangleq  \begin{bmatrix} \nabla_{x} J_e(x,u)\rvert_{\begin{subarray}{l}x=x_l(s_1) \\ u=u_l(s_1)\end{subarray}} \\
    \vdots\\
    \nabla_{x} J_e(x,u)\rvert_{\begin{subarray}{l}x=x_l(s_{n_s}) \\ u=u_l(s_{n_s})\end{subarray}}
    \end{bmatrix}^T Q_{sx},
\end{equation}
where $Q_{sx}$ is a diagonal weighting matrix designed to weight and also normalize the states in the overall performance.

The performance index of \eqref{eqn:longFormPerformance} can now be written in an equivalent super-block structure using the super-lifted vectors $\mathbf{u}_{j+1}$, and $\mathbf{u}_{j+1}$:
\begin{equation}\label{eqn:superBlockPerformance}
\begin{split}
\mathbf{J}_{j+N} = 
& \mathbf{u}_{j+1}^T \mathbf{Q_u} \mathbf{u}_{j+1} + \mathbf{u}_{j+1}^T \mathbf{D}_u^T \mathbf{Q_{\delta u}} \mathbf{D}_u \mathbf{u}_{j+1} \\
&+ \left(\mathbf{E}_u\mathbf{u}_{j+1}-u_j\right)^T Q_{\delta u} \left(\mathbf{E}_u\mathbf{u}_{j+1}-u_j\right)\\
&+ \mathbf{x}_{j+1}^T \mathbf{Q_x} \mathbf{x}_{j+1} + \mathbf{x}_{j+1}^T \mathbf{D}_x^T \mathbf{Q_{\delta x}} \mathbf{D}_x \mathbf{x}_{j+1} \\
&+ \left(\mathbf{E}_x\mathbf{x}_{j+1}-x_j\right)^T Q_{\delta x} \left(\mathbf{E}_x\mathbf{x}_{j+1}-x_j\right)\\
&+ \mathbf{e}_{j+1}^T \mathbf{Q_e} \mathbf{e}_{j+1} + \mathbf{e}_{j+1}^T \mathbf{D}_e^T \mathbf{Q_{\delta e}} \mathbf{D}_e \mathbf{e}_{j+1} \\
&+ \left(\mathbf{E}_e\mathbf{e}_{j+1}-e_j\right)^T Q_{\delta e} \left(\mathbf{E}_e\mathbf{e}_{j+1}-e_j\right)\\
&+ \mathbf{S_x}\mathbf{x}_{j+1}
\end{split}
\end{equation}
where $\mathbf{D}_u\in \mathbb{R}^{(N_i-1) n_s n_u\times N_i n_s n_u}$, $\mathbf{D}_x\in \mathbb{R}^{(N_i-1) n_s n_u\times N_i n_s n_u}$, and $\mathbf{D}_e \in \mathbb{R}^{(N_i-1) n_s n_u\times N_i n_s n_u}$ are difference operator matrices designed to calculate the difference between sequences during subsequent iterations according to 
\begin{equation}
    \mathbf{D}_{(\cdot)} = \begin{bmatrix}
    \mathbb{I} & -\mathbb{I} & \mathbb{0} & \hdots\\
    \mathbb{0} & \mathbb{I} & -\mathbb{I} &  \hdots\\
    \vdots & \vdots & \vdots & \ddots
    \end{bmatrix},
\end{equation}
where the identity matrix has dimensions of $n_{(\cdot)} n_s \times n_{(\cdot)} n_s$.  Note that $\mathbf{D}_{(\cdot)}$ has $N_i-1$ block rows and $N_i$ block columns.  Additionally, the matrices $\mathbf{E}_u$, $\mathbf{E}_u$, and $\mathbf{E}_u$ are defined in such as way as to select the first lifted vector from the super-vector.  Specifically, 
\begin{equation}
    \mathbf{E}_{(\cdot)}\triangleq \begin{bmatrix} \mathbb{I}^{n_{(\cdot)} n_s \times n_{(\cdot)} n_s} & \mathbb{0}^{n_{(\cdot)} n_s \times (N_i-1) n_{(\cdot)} n_s} \end{bmatrix}.
\end{equation}
By using \eqref{eqn:superLiftedModel} in \eqref{eqn:liftedError} and \eqref{eqn:superBlockPerformance}, we can obtain an expression for the performance index completely in terms of the known quantities from the last iteration, $\underline{u}_j$, and $\underline{x}_j$, along with the control sequences over the next several iterations, $\mathbf{u}_{j+1}$.  By then differentiating this expression for performance, $\mathbf{J}_{j+1}$ with respect to the elements of $\mathbf{u}_{j+1}$, setting the result equal to the zero vector, and re-arranging the resulting expression, we obtain an update law of the form 
\begin{align}
\mathbf{u}_{j+1} & = L_u u_j + L_e e_j + L_x x_j + L_c,
\end{align}
where
\begin{align}
L_0 & \triangleq \left(\mathbf{\hat{Q}_u} + \mathbf{G}_j^T \left(\mathbf{\hat{Q}_x} + \mathbf{\hat{Q}_e} \right)\mathbf{G}_j \right)^{-1}\\
L_u & \triangleq L_0\left(\mathbf{E}_u^T Q_{\delta u} + \mathbf{G}_j^T \left(\mathbf{\hat{Q}_x} +  \mathbf{\hat{Q}_e} \right) \mathbf{G}_j \mathbf{I}_u \right)\\
L_x & \triangleq L_0\mathbf{G}_j^T\left(\mathbf{E}_x^T Q_{\delta x} - \mathbf{\hat{Q}_x} \mathbf{I}_x  - \mathbf{\hat{Q}_x} \mathbf{F}_j  - \mathbf{\hat{Q}_e} \mathbf{F}_j \right)\\
L_e & \triangleq L_0 \mathbf{G}_j^T \left( \mathbf{\hat{Q}_e} \mathbf{I}_e - \mathbf{E}_e^T Q_{\delta e} \right)\\
L_c & \triangleq -\frac{1}{2}L_0\mathbf{G}_j^T\mathbf{S}_x^T
\end{align}
and
\begin{align}
    \mathbf{\hat{Q}_u} & \triangleq \mathbf{Q_u} + \mathbf{D}_u^T\mathbf{Q_{\delta u}} \mathbf{D}_u + \mathbf{E}_u^T Q_{\delta u} \mathbf{E}_u\\
    \mathbf{\hat{Q}_x} & \triangleq \mathbf{Q_x} + \mathbf{D}_x^T\mathbf{Q_{\delta x}} \mathbf{D}_x + \mathbf{E}_x^T Q_{\delta x} \mathbf{E}_x \\
    \mathbf{\hat{Q}_e} & \triangleq \mathbf{Q_e} + \mathbf{D}_e^T\mathbf{Q_{\delta e}} \mathbf{D}_e + \mathbf{E}_e^T Q_{\delta e} \mathbf{E}_e.
\end{align}

It should be emphasized here that this update law produces the super-lifted vector $\mathbf{u}_{j+1}$, which contains control sequences for multiple future iterations.  Thus, while it would be technically possible to perform multiple iterations based on this single update law, we choose to only run a single iteration before performing this update again.  This is justified by the same reasons that are usually cited for model predictive control (MPC).  By updating the the control sequence after every iteration, we incorporate the most recent information, making the system more robust to disturbances and modeling uncertainties.  We describe the resulting control structure as iteration-domain receding horizon control or receding horizon iterative learning control (RHILC).

